Polarization and Belief Convergence of Agents in Strongly-Connected Influence Graphs

We describe a model for polarization in multi-agent systems based on Esteban and Ray's classic measure of polarization from economics. Agents evolve by updating their beliefs (opinions) based on the beliefs of others and an underlying influence graph. We show that polarization eventually disappears (converges to zero) if the influence graph is strongly-connected. If the influence graph is a circulation we determine the unique belief value all agents converge to. For clique influence graphs we determine the time after which agents will reach a given difference of opinion. Our results imply that if polarization does not disappear then either there is a disconnected subgroup of agents or some agent influences others more than she is influenced. Finally, we show that polarization does not necessarily vanish in weakly-connected graphs, and illustrate the model with a series of case studies and simulations giving some insights about polarization.

==> general-case.tex <==
%\todo{M\'ario: I moved this into an appendix for the time being, since we agreed these results won't go into the Fossacs paper.}
If we look at the condensation graph of our influence graph, we will see that there are vertices (which represent strongly connected components of the original graph) which do do not have any edges leading to them (since the condensed graph is a directed acyclic graph). These vertices represent strongly connected components that do not receive external influence and, thus, converge according to Theorem \ref{theorem:scc-convergence}.

%\todo {This does not follow immediately due to constant factors, since the full graph is larger and, thus, changes $|\Agents|$, we should either do a more general proof or show this case.}

\begin{figure}[h!]
    \centering
    \scalebox{0.8}{
        \begin{tikzpicture}
            \tikzstyle{every state}=[fill opacity=1,text opacity=1,semithick,minimum size=10pt]
            
            \node[state] (0) [fill=red1]                 {{\color{White}0}};
            \node[state] (1) [below left of=0, fill=red1]                 {{\color{White}1}};
            \node[state] (2) [below right of=0, fill=red1]                {{\color{White}2}};
            \node[state] (3) [below left of=1, fill=green1]                 {{\color{White}3}};
            \node[state] (4) [below right of=2, fill=RoyalBlue]                 {{\color{White}4}};
            \node[state] (5) [below right of=4, fill=RoyalBlue]                {{\color{White}5}};
            \node[state] (6) [below left of=3, fill=BurntOrange]                 {{\color{White}6}};
            \node[state] (7) [below right of=3, fill=BurntOrange]                 {{\color{White}7}};
            
            \draw
            (0) edge[->,thick,bend left=15]  (1)
            (0) edge[->,thick,bend left=15]  (2)
            (2) edge[->,thick,bend left=15]  (0)
            (2) edge[->,thick,bend left=15]  (1)
            (1) edge[->,thick,bend left=15]  (0)
            (1) edge[->,thick,bend left=15]  (2)
            (3) edge[->,thick,left]   (1)
            (6) edge[->,thick,left]   (3)
            (6) edge[->,thick,bend left=15]  (7)
            (7) edge[->,thick,bend left=15]  (6)
            (4) edge[->,thick]   (2)
            (4) edge[->,thick,bend left=15]  (5)
            (5) edge[->,thick,bend left=15]  (4)
            (7) edge[->,thick,left]   (3)
            ;
        \end{tikzpicture}
    }
\end{figure}

\begin{figure}[h!]
    \centering
    \scalebox{1}{
        \begin{tikzpicture}
            \tikzstyle{every state}=[fill opacity=1,text opacity=1,semithick,minimum size=26pt]
            
            \node[state] (0) [fill=red1]                 {\color{White}0,1,2};
            \node[state] (1) [below left of=0, fill=green1]                 {\color{White}3};
            \node[state] (2) [below right of=0, fill=RoyalBlue]                {{\color{White}4,5}};
            \node[state] (3) [below left of=1, fill=BurntOrange]                 {{\color{White}6,7}};

            \draw
            (1) edge[->,thick,left]   (0)
            (3) edge[->,thick,left]   (1)
            (2) edge[->,thick,left]   (0)
            ;
        \end{tikzpicture}
    }
    \caption{Condensation Graph} \label{fig:condensation-graph}
\end{figure}

\begin{lemma}\label{lemma:scc-path}
Every SCC either converges according to Theorem \ref{theorem:scc-convergence} (by having no edge that reaches it in the condensed graph) or there is a path from an SCC that converges to it.
\end{lemma}

We leave the proof to the reader. 

%\begin{proof}
%Suppose that the SCC has edges reaching it and we are going to prove, by contradiction, that there must be a path from a SCC that converges to it.
%Looking at the condensation graph, there is a vertex that leads to the vertex $v$ that represents our SCC, this vertex cannot converge, by hypothesis, thus it also has a vertex that leads to it. We can repeat this procedure infinitely and we would end up either with an infinite graph or with a cycle, and both of them are contradictions.
%\end{proof}

Since some components converge and do not depend on the rest of the components, we can replace their beliefs by their limit beliefs and remove the internal edges. Because our belief update functions are continuous, this change does not change the convergence and limit value of other components, even though it may increase the speed of convergence.% \emph{w.l.o.g.} 
%\todo{How to show that this does not matter when talking about belief convergence? Sophia: I added some details.}
(in respect to belief convergence).

\begin{figure}[h!]
    \centering
    \scalebox{0.75}{
        \begin{tikzpicture}
            \tikzstyle{every state}=[fill opacity=1,text opacity=1,semithick,minimum size=10pt]
            
            \node[state] (0) [fill=red1]                 {{\color{White}0}};
            \node[state] (1) [below left of=0, fill=red1]                 {{\color{White}1}};
            \node[state] (2) [below right of=0, fill=red1]                {{\color{White}2}};
            \node[state] (3) [below left of=1, fill=green1]                 {{\color{White}3}};
            \node[state] (4) [below right of=2, fill=Black]                 {{\color{White}4}};
            \node[state] (5) [below right of=4, fill=Black]                {{\color{White}5}};
            \node[state] (6) [below left of=3, fill=Black]                 {{\color{White}6}};
            \node[state] (7) [below right of=3, fill=Black]                 {{\color{White}7}};
            
            \draw
            (0) edge[->,thick,bend left=15]  (1)
            (0) edge[->,thick,bend left=15]  (2)
            (2) edge[->,thick,bend left=15]  (0)
            (2) edge[->,thick,bend left=15]  (1)
            (1) edge[->,thick,bend left=15]  (0)
            (1) edge[->,thick,bend left=15]  (2)
            (3) edge[->,thick,left]   (1)
            (6) edge[->,thick,left]   (3)
            (7) edge[->,thick,left]   (3)
            (4) edge[->,thick]   (2)
            ;
        \end{tikzpicture}
    }
\end{figure}

\begin{lemma}
$\forall \agent{i},\agent{j} \in \Agents$ there are constants $\IfunR{\agent{j}}{\agent{i}}$ such that $\underset{\agent{j} \in \Agents}{\sum}\IfunR{\agent{j}}{\agent{i}} = 1$ and for all $t$,
$$\Bfun{\agent{i}}{t+1} = \underset{\agent{j} \in \Agents}{\sum} \IfunR{\agent{j}}{\agent{i}}\Bfun{\agent{j}}{t}$$  
%\todo{Sophia added "for all $t$ for clarity.}
\end{lemma}

\begin{proof}
We can construct the constants by normalizing influence by number of agents:
\begin{equation*}
    \IfunR{\agent{j}}{\agent{i}} = 
    \begin{cases} 
       \frac{1}{|\Agents|}\Ifun{\agent{j}}{\agent{i}}, &  i \neq j \\
      1 - \frac{1}{|\Agents|}\underset{\agent{j} \in \Agents \setminus \{\agent{i}\}}{\sum}\Ifun{\agent{j}}{\agent{i}}, & i = j
   \end{cases}
\end{equation*}

Clearly they sum up to $1$, now we shall prove that:

\begin{align*}
    \Bfun{\agent{i}}{t+1} = \underset{\agent{j} \in \Agents}{\sum} \IfunR{\agent{j}}{\agent{i}}\Bfun{\agent{j}}{t}
\end{align*}

According to Equation \ref{eq:symplification}:

\begin{align*}
    \Bfun{\agent{i}}{t+1} &= \Bfun{\agent{i}}{t} + \frac{1}{|\Agents|}\underset{\agent{j} \in \Agents}{\sum} \Ifun{\agent{j}}{\agent{i}}(\Bfun{\agent{j}}{t}-\Bfun{\agent{i}}{t}) \\
    &= \Bfun{\agent{i}}{t} + \frac{1}{|\Agents|}\underset{\agent{j} \in \Agents\setminus \{\agent{i}\}}{\sum} \Ifun{\agent{j}}{\agent{i}}(\Bfun{\agent{j}}{t}-\Bfun{\agent{i}}{t}) \ \ \ \  %\text{(Lemma 4)}
    \\
    &= \Bfun{\agent{i}}{t}(1-\frac{1}{|\Agents|}\underset{\agent{j} \in \Agents\setminus \{\agent{i}\}}{\sum}\Ifun{\agent{j}}{\agent{i}}) + \frac{1}{|\Agents|}\underset{\agent{j} \in \Agents\setminus \{\agent{i}\}}{\sum} \Ifun{\agent{j}}{\agent{i}}\Bfun{\agent{j}}{t}\\
    &= \Bfun{\agent{i}}{t}(1-\underset{\agent{j} \in \Agents\setminus \{\agent{i}\}}{\sum}\frac{1}{|\Agents|}\Ifun{\agent{j}}{\agent{i}}) + \underset{\agent{j} \in \Agents\setminus \{\agent{i}\}}{\sum} \frac{1}{|\Agents|}\Ifun{\agent{j}}{\agent{i}}\Bfun{\agent{j}}{t}\\
   % &= \Bfun{\agent{i}}{t}(1-\underset{\agent{j} \in \Agents\setminus \{\agent{i}\}}{\sum}\IfunR{\agent{j}}{\agent{i}}) + \underset{\agent{j} \in \Agents\setminus \{\agent{i}\}}{\sum} \IfunR{\agent{j}}{\agent{i}}\Bfun{\agent{j}}{t}\\
    &= \IfunR{\agent{i}}{\agent{i}}\Bfun{\agent{i}}{t} + \underset{\agent{j} \in \Agents\setminus \{\agent{i}\}}{\sum} \IfunR{\agent{j}}{\agent{i}}\Bfun{\agent{j}}{t}\\
    &= \underset{\agent{j} \in \Agents}{\sum} \IfunR{\agent{j}}{\agent{i}}\Bfun{\agent{j}}{t}
\end{align*}

Since every belief is composed of a linear combination of other beliefs multiplied by constants, we can write the belief update as a matrix multiplication:

Calling $B^t_v$ the \emph{belief vector in the time $t$}, in which the $i$\textsuperscript{th} entry represents the belief of agent $\agent{i}$, we want a matrix $M$ that satisfies $M.B^t_v = B^{t+1}_v$. It is clear that, $M_{i,j} = \IfunR{\agent{j}}{\agent{i}}$ satisfies those properties, thus we will call $M$ the \emph{update matrix}.

We showed that the real influences sum up to one and are positive, so the update matrix is a Markov matrix, since its rows sum to one. 
%\todo{Sophia:my changes start here }
And we note that in the influence graph corresponding to the update matrix, the weights of the \emph{incoming} transitions to any state sum to 1, and therefore this graph is the transpose of the graph of a Markov model, where all outgoing transitions must sum to 1. Recall that we are considering the condensation graph of the original system, and in the condensation graph, the nodes with no incoming transitions represent connected components which are guaranteed to converge. Thus, in the transposed graph, each node with no outgoing transitions represents a connected component, guaranteed to converge. We will call these vertices leaves. Furthermore, from Lemma \ref{lemma:scc-path}, each vertex in the transposed graph which is not a leaf has a path to a leaf.  

The influence graph that it represents, when multiplied by the left, is equivalent to the transposed graph 
%\todo{This is the weird part of the argument, I do not know how to formalize it, but it makes sense since by the right-hand side each state is composed by the lines and, by the left-hand side, each state is composed by the columns.}
and, in this graph, according to Lemma \ref{lemma:scc-path}, each vertex either has converged or has a path to a converged state (since we are looking at the transposed graph). The agents $\agent{i}$ that converged have $\IfunR{\agent{i}}{\agent{i}} = 1$, since we took out every other edge inside the SCC. Thus, the update matrix is, in fact, an absorbing Markov chain 
%\todo{How to be more formal defining this matrix?}. 
Now that we have those properties, belief convergence can be stated as the existence of the limit:

\begin{align*}
    \underset{t \to \infty}{\lim} M^tB_v^0
\end{align*}

It is sufficient, although not necessary, that the limit: $\underset{t \to \infty}{\lim} M^t$ exists to guarantee the existence of the one above. Since $M$ is an absorbing Markov chain, the limit exists according to 
%\todo{We need to cite a proof on this fact}.

\begin{theorem}\label{theorem-general-belief-conversion}
$\forall \agent{i} \in \Agents, \exists L \in \R$ such that $ \underset{t \to \infty}{\lim} \Bfun{i}{t} = L$.
\end{theorem}

\end{proof}
